Geodesic interpolation of frame-wise speaker embeddings for the diarization of meeting scenarios

We propose a modified teacher-student training for the extraction of frame-wise speaker embeddings that allows for an effective diarization of meeting scenarios containing partially overlapping speech. To this end, a geodesic distance loss is used that enforces the embeddings computed from regions with two active speakers to lie on the shortest path on a sphere between the points given by the d-vectors of each of the active speakers. Using those frame-wise speaker embeddings in clustering-based diarization outperforms segment-level clustering-based diarization systems such as VBx and Spectral Clustering. By extending our approach to a mixture-model-based diarization, the performance can be further improved, approaching the diarization error rates of diarization systems that use a dedicated overlap detection, and outperforming these systems when also employing an additional overlap detection.

==> tikz/geodesic.tex <==
\begin{tikzpicture}
\node[coordinate] (start) {};
\node[coordinate, above=2cm of start] (d1) {};
\node[coordinate, right=2cm of start] (d2) {};
%
\draw[->] (start) -- node[near end] {$\mathbf{d}_1$} (d1);
\draw[->] (start) -- node[near end] {$\mathbf{d}_2$} (d2),
\draw[-] (d1) -- (d2) {};
\path [red,bend left,line]   (d1) edge (d2);

\end{tikzpicture}
